Measuring D\'ej\`a vu Memorization Efficiently

Recent research has shown that representation learning models may accidentally memorize their training data. For example, the d\'ej\`a vu method shows that for certain representation learning models and training images, it is sometimes possible to correctly predict the foreground label given only the representation of the background - better than through dataset-level correlations. However, their measurement method requires training two models - one to estimate dataset-level correlations and the other to estimate memorization. This multiple model setup becomes infeasible for large open-source models. In this work, we propose alternative simple methods to estimate dataset-level correlations, and show that these can be used to approximate an off-the-shelf model's memorization ability without any retraining. This enables, for the first time, the measurement of memorization in pre-trained open-source image representation and vision-language representation models. Our results show that different ways of measuring memorization yield very similar aggregate results. We also find that open-source models typically have lower aggregate memorization than similar models trained on a subset of the data. The code is available both for vision and vision language models.

==> introduction.tex <==
\section{Introduction}

Representation learning has emerged as one of the major pillars of computer vision. The goal in representation learning is to learn a model that produces semantically meaningful representations, where images or image-text pairs that are close in meaning occur close together in representation space. These learned representations can then be used in numerous downstream applications such as semantic segmentation~\citep{kirillov2023segany}, image generation~\citep{rombach2022high} and multi-modal LLMs~\citep{liu2024visual}.
A natural question that arises is whether these representation learning models memorize their training data and to what extent. Excessive memorization may call the generalization abilities of the models into question. In addition, if the models are trained on confidential data, then memorization might also lead to leakage of confidential information from the models. Thus, there is a need to develop a way to measure if memorization is taking place.

Since learned representations are usually abstract and hard to interpret, memorization measurement for representation learning models requires careful design.
Currently, a standard way of doing this is the \dejavu method, which designs a causal task of predicting parts of the training sample given another disjoint part, and uses performance on this task to determine if the model memorizes. For example, \citet{Dejavu} designed the task of predicting the foreground object given the background crop of a training image, as shown in \autoref{fig:intro_figure} (orange block). Achieving a high performance on this task indicates two possibilities: \emph{(i)} if the model has memorized the association of the background crop with the foreground object for a specific training sample, or \emph{(ii)} if the model has learned the dataset-level correlation between the background crop and a given foreground object. To rule out the second possibility, \citet{Dejavu} opted for a two-model approach, training two separate models on disjoint parts of the training set and using the gap in performance between the two models as indication of memorization. This approach has been extended by \citet{jayaraman2024deja} to measure memorization of vision-language models such as CLIP~\citep{radford2021learning}.

Despite the success of the \dejavu method in defining and measuring memorization, scaling this approach to state-of-the-art representation learning models is challenging. First of all, the two-model approach requires the model trainer to split the training set into disjoint halves, which severely constrains the valuable training data. Moreover, even if data is abundant, training the second model on internet-scale datasets is computationally expensive. Due to these limitations, the \dejavu test cannot be used to measure memorization of pre-trained models out-of-the-box.

In this work, we provide simple alternative ways of quantifying dataset-level correlations and show that they suffice for the purpose of measuring \dejavu memorization. Specifically, for image representation learning, we propose two alternative ways to derive reference models to predict the foreground label from a background crop: training an image classification network directly, and using a Naive Bayes classifier on top of a pre-trained object detection model. We then leverage these reference models to define a \emph{one-model} \dejavu test---a memorization test for representation learning models that only requires training a simpler reference model \emph{once per dataset}. \autoref{fig:intro_figure} (green block) gives an illustration of our proposed one-model \dejavu test. We also propose a variant of the method for vision-language models by leveraging a pre-trained text embedding model.

We validate our proposed methods by comparing them to the two-model test on ImageNet-trained image representation learning models, as well as CLIP models trained on a privately licensed image-caption pair dataset. We find that the one-model test can successfully identify memorized examples and obtain similar population-level memorization scores as the two-model test. We also evaluate the one-model \dejavu test on pre-trained open-source models and show that it can be used out-of-the-box to identify samples that are likely memorized by the model. We advocate our one-model test as a practical tool for debugging memorization of representation learning models.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/DejaVu1Model_4.pdf}
    \caption{Illustration of our one-model \dejavu test for image representation learning. The task is to predict the foreground object given a background crop. The original \dejavu test~\citep{Dejavu} trains two models $\text{SSL}_A$ and $\text{SSL}_B$ on disjoint splits of the training set, and uses $\text{SSL}_B$ to quantify the degree of dataset-level correlation between the foreground and background crop. Our one-model test replaces $\text{SSL}_B$ with a classifier that directly predicts the foreground given background crop, and we show that both ResNet50 network and Naive Bayes classifier work well for this purpose.}
    \label{fig:intro_figure}
    \vspace{-2ex}
\end{figure}

%\chuan{TODO: one short paragraph about experiments}

%\narine{Describe why we call our method One Model Test despite that we use two models. @Chuan I have a short paragraph about it here \ref{onemodel} but we might want to describe it sooner in the introduction.}

\begin{comment}
% First, explain what DejaVu is
\Dejavu was introduced by \citet{Dejavu} who demonstrated that SSL methods on image datasets can memorize their training data. This setup was based on the premise that SSL models are trained to map different crops of a given image to similar embedding in the representation space of the model. Thus, from partial information like a background crop of a given image that does not contain the class labelled object of interest, a model could potentially retrieve the correct class information. This can happen either if the model has memorized that the background crop should be associated with a given object or if a model has learned that the background crop is often correlated with a given object. To differentiate those two scenarios of leveraging correlations versus memorizing the training data, the authors introduced an experimental setup with two models. Each of them was trained on different non-overlapping subset of a given dataset. If both models were able to predict the correct class for a given image (which was part of the training set of the first model, but not on the second model), then the authors assumed that it was because of correlations. If the first model was able to predict the correct class while the second model was not able to, then the authors considered that this was an instance of memorizing the training data. Following work by \citet{jayaraman2024deja} extended \dejavu to Vision-Language-Model (VLMs). Instead of leveraging a background crop, the authors use a given caption to retrieve information from a training data image. By also using two models, one which was trained using given test caption-images pairs, and one which was not using those pairs, they were able to assess if a model ability to predict the correct image from the caption was due to correlation or memorization.

However, both approaches require to train from scratch two models to differentiate correlation from memorization. This also mean that such techniques require to train models on non-overlapping subsets of data which significantly reduce the amount of training data by models. Most models that are open-source are trained on the full datasets and retraining them even on a subset can be costly. This raise the main question of this paper which is: How to quantify memorization on a given open-source model without having to retrain it? One hypothesis we had to answer this question was that the correlations, a model is able to exploit at the image level to predict the correct class given only the background, are not really model dependent. The correlations are just an artefact on how the dataset was built and the long-tail nature of real data. 

By discovering which are the correlations associated with a given dataset, then we can approximate how much a given model memorized by just removing the correlated data points. In this paper, we are introducing two simple techniques to discover correlations in the training data. One can use a naive bayes approximation to assess how much specific objects in an image are correlated with each others. We can also train a classifier on background crop and see which classes are correctly classified. We evaluate how close the classes affected by correlations found with this technique are from the original work of \citet{Dejavu}.

After finding those correlations, we measure how strong the memorization is on open-source models with respect to the baseline in \citet{Dejavu}. Then, we extend this one model approach to VLMs following the setup from \citet{jayaraman2024deja}. In that instance, we replace the use of the naive Bayes classifier or a resnet by a Large-Language-Model (LLM) to find the correlations in the captions. If the LLM is able to guess correctly which are the correlated factors associated to a given caption, then the VLM is able to retrieve the correct images because of correlations. If it is not the case, then we can say it is because of memorization. 
\end{comment}

\paragraph{Contributions.} To summarize, our main contributions are as follows:
\begin{enumerate}[leftmargin=*]
    \item We develop simple and efficient methods to quantify dataset-level correlations for both image-only and vision-language representation learning models. Our methods enable \dejavu memorization tests without training two models on disjoints splits of the training set.
    \item We validate our proposed methods by comparing them to the two-model test, and analyze the strengths and weaknesses of both tests.
    \item We evaluate the one-model \dejavu test on open-source image-only and vision-language representation models. Our test reveals that open-source models do memorize specific training samples, but overall to a lesser degree than the same model trained on smaller subsets of data. We plan to release our code and a list of top dataset-level correlations upon public release of the paper.% Our evaluation shows that open source pre-trained models memorize substantial amount of data but less than the same models trained on smaller subsets of data.
\end{enumerate}

\iffalse
\begin{itemize}
\item introduce deja vu memorization

\item main way to do deja vu memorization is in two steps -- first, we find a task that cannot be done causally (eg, predict foreground from background); second, this could also happen through spurious correlations, so we rule out spurious correlations through a second model. 

\item However, this makes it infeasible to run on models in the wild. One way would be to retrain a second model on a disjoint data set -- this is too hard because there is not enough disjoint data. The other way is to retrain a model on the entire training data minus one or a few points -- that does not scale in terms of compute. 

\item in this work, we investigate how to do this by using a single model so that the measurement techniques scale to the larger models of today. 

\end{itemize}
\fi

==> outline.tex <==
Measuring Deja Vu Memorization Efficiently

Representation learning has emerged as one of the major pillars of computer vision. Given a training dataset, the goal is to learn a model that produces semantically meaningful representations -- where images or image-text pairs that are close in meaning occur close together in representation space. These representations can then be used in numerous applications, such as ....

A natural question that arises is whether these representation learning models memorize their training data and to what extent. Excessive memorization may call the generalization abilities of the models into question. In addition, if the models are trained on sensitive data, then memorization might also lead to leakage of sensitive information from the models. Thus, there is a need to develop a way to measure if memorization is taking place.

A standard way of measuring memorization in representation learning is the \dejavu method. (say what it is -- there is a task that cannot be causally done, and a way to rule out if this can be done through dataset-level correlations.) Prior work selected task X. To rule out dataset level correlations, they used a second model ... However, a major barrier to scaling .. is the second model -- ...

In this work, we provide simple alternative ways of measuring dataset-level correlations and we show that they suffice for the purpose of measuring memorization. Specifically, for images, .... (describe in a couple of sentences). We also provide a version of the method for vision-language models.

one short paragraph about experiments

